GraphAD: A Graph Neural Network for Entity-Wise Multivariate Time-Series Anomaly Detection

In recent years, the emergence and development of third-party platforms have greatly facilitated the growth of the Online to Offline (O2O) business. However, the large amount of transaction data raises new challenges for retailers, especially anomaly detection in operating conditions. Thus, platforms begin to develop intelligent business assistants with embedded anomaly detection methods to reduce the management burden on retailers. Traditional time-series anomaly detection methods capture underlying patterns from the perspectives of time and attributes, ignoring the difference between retailers in this scenario. Besides, similar transaction patterns extracted by the platforms can also provide guidance to individual retailers and enrich their available information without privacy issues. In this paper, we pose an entity-wise multivariate time-series anomaly detection problem that considers the time-series of each unique entity. To address this challenge, we propose GraphAD, a novel multivariate time-series anomaly detection model based on the graph neural network. GraphAD decomposes the Key Performance Indicator (KPI) into stable and volatility components and extracts their patterns in terms of attributes, entities and temporal perspectives via graph neural networks. We also construct a real-world entity-wise multivariate time-series dataset from the business data of Ele.me. The experimental results on this dataset show that GraphAD significantly outperforms existing anomaly detection methods.

==> src/dataset.tex <==
\subsection{Dataset}
\subsubsection{Background}
We construct a dataset from transaction data in Ele.me, which is a representative scene for entity-wise multivariate time-series anomaly detection. Raw data consist of transaction records between retailers and consumers from Jun. 30th, 2020 to Jun. 30th, 2021, containing desensitized information about consumers, retailers and couriers. There are 70 attributes in one record, including order details like pay amount, delivery time and distance. 

\subsubsection{Preprocessing}


To avoid the time alignment problem caused by missing records on different days for various retailers, we choose retailers that sell goods every day during the selected duration. Besides, anomaly detection for retailers with low turnover is worthless from the industry perspective, so we filter out retailers whose average daily transaction records are less than 20. 
The data are organized as $X\in\mathbb{R}^{N\times T\times D}$ where $N$ is the number of retailers, $T$ is the number of days and $D$ is the attribute dimension. We aggregate numeric attributes of daily records in average or summation form, while category attributes are counted by values. We also take into account the impact of couriers; for example, couriers delivering food at lower speed are more likely to raise transaction issues. Hence, we design couriers-related attributes like "# order delivery on time". Finally, we obtain 114 attributes for each retailer each day. The corresponding labels are generated based on $X$ and business requirements.

Given the static similarity between retailers, we also extract static retailer attributes such as "open time", "product type" and "location". And our goal is to use 30 days of data to decide the operating condition on the 31st day.

\subsubsection{Data Distribution}
We detail the dataset to provide intuition on the scene of Ele.me. From the perspective of delivery, the number of orders sent to consumers ahead of time follows the Gaussian distribution, while the overtime orders follow a uniform distribution. The total number of the abnormal day varies across retailers with the majority being three.
The number of retailers with a total number of abnormal days less than 7 takes up more than 80$\%$ of the data, revealing the long-tail distribution of the dataset.
